Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution

With music becoming an essential part of daily life, there is an urgent need to develop recommendation systems to assist people targeting better songs with fewer efforts. As the interactions between users and songs naturally construct a complex network, community detection approaches can be applied to reveal users' potential interests on songs by grouping relevant users & songs to the same community. However, as the types of interaction could be heterogeneous, it challenges conventional community detection methods designed originally for homogeneous networks. Although there are existing works on heterogeneous community detection, they are mostly task-driven approaches and not feasible for specific music recommendation. In this paper, we propose a genetic based approach to learn an edge-type usefulness distribution (ETUD) for all edge-types in heterogeneous music networks. ETUD can be regarded as a linear function to project all edges to the same latent space and make them comparable. Therefore a heterogeneous network can be converted to a homogeneous one where those conventional methods are eligible to use. We validate the proposed model on a heterogeneous music network constructed from an online music streaming service. Results show that for conventional methods, ETUD can help to detect communities significantly improving music recommendation accuracy while simultaneously reducing user searching cost.

==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/conclusion.tex <==
\section{Conclusion}
 \vspace{-1em}
In this paper, we put efforts on how to convert a heterogeneous network to a homogeneous one so that conventional community detection methods can still be eligible to use. It extends the application scope of those conventional methods and endows them more generalizable and robust usage. To achieve this, a genetic based approach is developed to learn the edge-type usefulness distribution (ETUD) on heterogeneous networks. Experiments on a real music dataset  show that involving ETUD in heterogeneous community detection is able to facilitate the accuracy of music recommendation with less search cost significantly. In the future, we will explore more sophisticated algorithms such as reinforcement learning methods for ETUD estimation. 
%In this paper, we propose a novel problem - \textit{heterogeneous graph community detection}, which provides important potential for graph-based search/recommendation where various kinds of nodes/edges available. A genetic approach is proposed to learn an optimized ETUD so as to convert a heterogeneous network to a homogeneous one. By doing that, the community detection algorithms, which originally designed only for homogeneous networks, are also able to generate reliable communities on large heterogeneous networks. In order to validate the performance of the proposed method, two retrieval tasks are applied on a dataset from a popular music online streaming service, Xiami. Experiment result showed that the learned ETUD can be an influential factor to solve the heterogeneous community detection problem. In the future, we will explore more sophisticated algorithm for ETUD estimation, while integrate this method to a graph embedding framework. Meanwhile, we will also investigate other retrieval/recommendation platforms, where heterogeneous data is available, to validate the proposed algorithm. 

%Future work should apply the same approach on other domains such as scholarly recommendation to verify whether our model is versatile and robust. Another potential track is     network pruning. As the types of relationships becomes complex, not all edge-types have equally important semantic meanings on the network. Hence, finding a better way to select edge-types can filter out the noises caused by unimportant edge-types and therefore generate better communities to solve recommendation/ retrieval tasks.

==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/copy.tex <==
\section{Results}

  \begin{table*}
        % \scriptsize
        \centering
    %   \vspace{-3em} 
    % \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|} \hline
        \multirow{2}{*}{\textbf{algorithm}} &  \multirow{2}{*}{\textbf{category}} & \multicolumn{2}{c}{\textbf{non edge-type learning}} & \multicolumn{2}{|c|}{\textbf{with edge-type learning $\alpha$ = 0.7}}  \\  
          &   & \textbf{cluster number}   &\textbf{searching cost} & \textbf{cluster number}   &\textbf{searching cost}         \\ \hline 
         deepWalk  &  embedding    &  100  &   3.6158   &  100  &  3.3958    \\ 
         LINE  &  embedding  &  100  &  2.5820    & 100   & 2.5211 \\ 
         node2vec    & embedding  &  100 &   3.8907   & 100   &  3.1776\\
         Louvain  &  modularity   & 12   &  3.8254   &  38  &    4.0254  \\ 
         Infomap  & random walk   &  3705  &   4.5357 &  4507  & 2.0513   \\ 
         BigClam    & overlapping  & 100  & 6.8448   &  100  &    4.8465\\
         \hline  
         \end{tabular}
         \caption{Search cost result comparison, search time cost is standardized}
         \label{tab:multiclass}
 \end{table*} 
 
 
 
 
 \begin{equation}
    Cost(u, S) = \sum_{s \in S}\mathbb{I}(G(u),G(s))\frac{C(u)*C(s)}{D(s|u)*\mu(\mathcal{N},\mathcal{C})^{2}} 
\end{equation}

C(u) and C(s) means the cluster size of user u and song s. $\mathcal{N}$ is the number of nodes in the graph, $\mathcal{C}$ is the number of communities. $\mu(\mathcal{N},\mathcal{C})$ is the average cluster size. D(s|u) is the preference degree of song s towards user u. $\mathbb{I}(u,s)$ is a judging function where:

\begin{equation}
  \mathbb{I}(G(u),G(s)) =
  \begin{cases}
    \alpha,       & \quad G(s) =  G(u)\\ 
    1-\alpha,  & \quad G(s) \neq  G(u)\\
  \end{cases}
  \label{eq:relu}
\end{equation}

$\alpha$ is from 0 to 1. G(s) refers to the community of s. 



  \begin{table*}
        % \scriptsize
        \centering
    %   \vspace{-3em} 
    % \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
       \textbf{algorithm} &  \textbf{category} & \textbf{edge-type weight} & \textbf{cluster number}   &\textbf{cost@5} &\textbf{cost@10}  &\textbf{cost@20}   &\textbf{cost@50}   &\textbf{cost@100}  \\ \hline 
         \multirow{2}{*}{DeepWalk}  &  \multirow{2}{*}{embedding}    &  No  &100    & 122.97   &   279.38 & 618.69  & 1562.37&3108.52\\ 
           &      &  Yes ($\alpha = 0.1$)  &  100 & 120.59   & 264.00   & 592.22  &1498.92 &2979.50\\ \hline 
         \multirow{2}{*}{LINE}  &  \multirow{2}{*}{embedding}    &  No  &100    &  95.62  &  213.37  & 456.83  & 1188.40&2298.26\\ 
           &      &  Yes ($\alpha = 0.1$)  & 100  & 91.45   &  211.23  & 444.95  & 1148.25&2227.35\\ \hline 
         \multirow{2}{*}{node2vec}  &  \multirow{2}{*}{embedding}    &  No  &   100 & 135.95   & 303.41   & 667.21  & 1698.62&3337.78\\ 
           &      &  Yes ($\alpha = 0.1$)  & 100  &  108.77  &  246.79  & 549.21  & 1385.76&2750.14\\ \hline 
        \multirow{2}{*}{Louvain}  &  \multirow{2}{*}{modularity}    &  No  & 38   &  2039.15  &  4240.29  & 9228.21  & 24045.29&47382.69\\ 
           &      &  Yes ($\alpha = 0.1$)  & 12  &  211.40  & 419.63   & 912.34  &2374.08 &4658.48\\ \hline 
         \multirow{2}{*}{Infomap}  &  \multirow{2}{*}{random walk}    &  No  &  3705  &  2.43E7   &   5.31E7 & 1.11E8  & 2.82E8&5.45E8\\ 
           &      &  Yes ($\alpha = 0.1$)  & 4507  & 1.68E7   &  3.52E7  & 7.25E7  &1.80E8 &3.51E8\\ \hline 
         \multirow{2}{*}{BigClam}  &  \multirow{2}{*}{overlapping}    &  No  &   100 &  4.47  &  19.80  & 55.59  &116.67 &193.59\\ 
           &      &  Yes ($\alpha = 0.1$)  & 100  & 3.00   &  8.77  &  19.17 & 41.52&82.80\\ \hline 
       
         \end{tabular}
         \caption{Search cost result comparison, search time cost is standardized}
         \label{tab:cost}
 \end{table*} 
 \begin{figure}
\subfloat[DeepWalk]{\includegraphics[width = 1.2in]{deepwalk.png}}
\subfloat[LINE]{\includegraphics[width = 1.2in]{line.png}}
\subfloat[node2vec]{\includegraphics[width = 1.2in]{node2vec.png}}\
\subfloat[Louvain]{\includegraphics[width = 1.2in]{louvain.png}} 
\subfloat[Infomap]{\includegraphics[width = 1.2in]{infomap.png}}
\subfloat[BigClam]{\includegraphics[width = 1.2in]{bigclam.png}} 
\caption{Tuning $\alpha$ of searching cost in six community detection algorithsm}
 \vspace{-1em}
 \label{fig:tune}
\end{figure} 
 

==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/data_copy.tex <==
\section{Data Preparation}

To test the effectiveness of the proposed approach, we collected a large dataset from an online music streaming system. Like many online music streaming services, the system allows users to play music on-demand, create and share playlists, bookmark and comment for their favorite artists and songs. In addition to bibliographical music metadata (artist, album, song, genre), we also collected the listening history of a large number of users, and other types of interaction these users performed on the service (the playlists they've created on the service, what artists/songs/albums they have bookmarked or commented on, etc.). The collected dataset contains 56,055 artists, 43,086 albums, 1,233,651 songs, 633 genres, 677,275 users, 305,916 playlists, and 15,879,347 relations between them. We randomly selected 500 users who have at least 50 songs in their listening history for test purpose. We use 60\% of the songs in their listening history to train the personal navigation profile, and the other 40\% are used for evaluation. We use another 500 users selected with the same criteria for global navigation profile training.

The heterogeneous music schema contains 6 types of nodes, and 32 types of edges (a relation and its reverse relation are considered belonging to two different edge types). We used a relatively simple heterogeneous graph with 6 types of edges for parameter tuning. The six edge types are artist-performsIn-song, album-includes-song, user-plays-song, and their reverse types.

In music recommendation domain, play count is generally considered a type of implicit feedback. Unlike explicit rating, the number of times a song is played is collected passively and contains a lot of noise (e.g. the user forgets to pause the player when her listening is interrupted) and does not accurately reflect the degree of preference from the user. It is generally agreed that the user listening to a song indicates the song appeals to her in some way, and the majority of the remaining songs in the catalog are less so. Thus, we use play counts as a binary indicator of whether the user has interest in a song, in all our experiments reported in this paper.
\begin{figure}[!htb]\centering
	\includegraphics[width=0.9\columnwidth]{paper/graphScheme.jpg}  
	\caption{Graph schema.}
	\label{fig:graph}
 \end{figure} %\vspace{-2em}



==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/evaluation.tex <==
\section{Experiment}
 \vspace{-1em}
\subsection{Dataset Description \& Parameter Setting}
 \begin{table}
%  \setlength{\abovecaptionskip}{-0.cm}
% \setlength{\belowcaptionskip}{-0.cm}
% \scriptsize
\centering
    %   \vspace{-3em} 
    \renewcommand{\tabcolsep}{3pt}
    \begin{tabular}{|l|l|l|l|l|l|} \hline
    \textbf{Node-type}   &\textbf{Count} & \textbf{Node-type}   &\textbf{Count}  &\textbf{Node-type}&\textbf{Count}       \\ \hline 
    
    Song& 54,353& User & 38,780& Genre& 543\\ \hline 
   Playlist &47,098 & Artist & 9,901& Album& 17,730\\ \hline 
 \end{tabular}
         \caption{Node statistics}
         \label{tab:node}
 \end{table} 
 
%   \begin{table}
% %  \setlength{\abovecaptionskip}{-0.cm}
% % \setlength{\belowcaptionskip}{-0.cm}
% % \scriptsize
% \centering
%     %   \vspace{-3em} 
%     \renewcommand{\tabcolsep}{3pt}
%     \begin{tabular}{|l|l|l|l|l|l|l|} \hline
%     \textbf{Node-type}   &Song & Playlist  & User & Artist&  Genre & Album\\ \hline 
    
%     \textbf{Number}& 54,353 & 47,098 & 38,780 & 9,901 & 543 & 17,730\\ \hline 
%  \end{tabular}
%          \caption{Node statistics}
%          \label{tab:node}
%  \end{table} 
 
 \begin{table}
        % \scriptsize
        \centering
%   \setlength{\abovecaptionskip}{-0.5cm}
% \setlength{\belowcaptionskip}{-0.cm}       
      \vspace{-1em} 
    \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|} \hline
    \textbf{Edge}   &\textbf{Name} & \textbf{Count}   & \textbf{Edge}   &\textbf{Name} & \textbf{Count}        \\ \hline 
    
    user$\to$song &plays &3,991,226 & user$\to$playlist&makes &42,775  \\ \hline 
    playlist$\to$song& includes& 514,652 &album$\to$song &include &40,798 \\ \hline 
    user$\to$artist&plays & 238,862& user$\to$artist&comment & 36,813\\ \hline 
    user$\to$song &bookmarks &213,602 &artist$\to$album &performsIn & 17,457\\ \hline
    user$\to$song&comments &136,078 & album$\to$genre&categorizedAs &15,174 \\ \hline
    user$\to$album&bookmarks &89,342 &user$\to$playlist &bookmark &9,982 \\ \hline 
    user$\to$album&comments & 59,575& artist$\to$genre& categorizedAs &9,726 \\ \hline 
    artist$\to$song&performsIn &57,675 &user$\to$playlist &comment &9443 \\ \hline 
 \end{tabular}
         \caption{Edge statistics}
         \label{tab:edge}
 \vspace{-2em} 
 \end{table} 

In this paper, the dataset used for music recommendation is from Xiami, one of the largest online music streaming services in China. Based on user behaviors and song profiles, a complex heterogeneous network is constructed. Details of the network are showed in Table \ref{tab:node} and Table \ref{tab:edge}. Besides this network, we also have all users listening history record as ground truth. For each user, all his/her listened songs are labelled as a score $\in \{1,2,3,4\}$, representing the quartile of their play counts belongs to. The listening history of 70 percent users are randomly sampled used to training our model ( used in Section 3.2), and the rest 30 percent users are used for our model validation.

%Thus, we use play counts as a categorical indicator of whether the user has interest in a song in all our experiments reported in this paper. This categorical indicator is within the range of \{1,2,3,4\}, representing each quartile of the play counts belongs to
%To validate the effectiveness of the proposed approach, we collected a large dataset from an online music streaming system, Xiami. Like many online music streaming services, the system allows users to play music on-demand, create and share playlists, bookmark and comment for their favorite artists and songs. In addition to bibliographical music metadata (artist, album, song, genre), we also collected the listening history of a large number of users, and other types of interaction these users performed on the service (the playlists they've created on the service, what artists/ songs/ albums they have bookmarked or commented on, etc.). In total, this heterogeneous music schema  (See Figure ~\ref{fig:graph}) contains 6 types of nodes, and 16 types of edges, which is shown in Table ~\ref{tab:node} and Table ~\ref{tab:edge}. 100 users who have at least 50 songs in their listening history are randomly selected for training purpose. Another 50 users with the same criteria are used for model evaluation.  

%For music recommendation, play count is generally considered a type of implicit feedback. Unlike explicit rating, the number of times a song is played is collected passively and contains a lot of noise (e.g. the user forgets to pause the player when her listening is interrupted) and does not accurately reflect the degree of preference from the user. It is generally agreed that the user listening to a song indicates the song appeals to him/her in some way, and the majority of the remaining songs in the catalog are less so. Thus, we use play counts as a categorical indicator of whether the user has interest in a song in all our experiments reported in this paper. This categorical indicator is within the range of \{1,2,3,4\}, representing each quartile of the play counts belongs to.

% \begin{figure}[!htb]\centering
% 	\includegraphics[width=0.9\columnwidth]{paper/graphScheme.jpg}  
% 	\caption{Music network schema}
% 	\label{fig:graph}
%  \end{figure} %\vspace{-2em}

%\subsection{ETUD optimization}
The parameters used in our approach are set based on empirical experiments and previous studies : number of initialized \emph{chromosome} $P$ = 1000; Cross-over threshold $t_c$ = 0.95 and Mutation threshold $t_m$ = 0.1; termination criteria is when the best \emph{chromosome} no longer changes for $\mathbb{N} = 10$ generations.

%\item initialized candidate number, $p$ = 100

%\item cross-over probability, $p(c)$ = 0.95

% \item cross-over exchange rate, $\alpha$ = 0.5

%\item mutation probability, $p(m)$ = 0.1

%\item number of iterations, $i$ = 500


\subsection{Searching Cost with Between-community Jumping} 
% To testify whether learned ETUD can really benefit music retrieval accuracy/efficiency as mentioned in the example case in Section Introduction, 50 users with their listening history are used to evaluate the retrieval performance of community structure with ETUD. 

The first task is to examine whether applying ETUD on heterogeneous networks can reduce the searching cost of retrieving all users' listened songs.  

In our music network, each user $u$ will belong to a community after a community detection method is leveraged. When user $u$ looks for songs to listen, there is a searching cost for the user to retrieve all his/her favored songs. We simulate user searching behaviours and define the overall searching cost as:

\begin{equation}
    Cost(U_{t}, S) = \sum_{u \in U_{t}}\sum_{k = 1}^{K}\sum_{s \in C_{u}^{k}}\frac{\sum_{s \in C_{u}^{k}}\mathbb{I}(s|u)}{\varphi(s|u)\sum_{s \in S}\mathbb{I}(s|u) }\cdot log(\lVert C_{u}^{(k-1)}\rVert \cdot \lVert C_{u}^{k}\rVert)  
    \label{eq:cost}
\end{equation}

$U_{t}$ is the collection of all testing users and $S$ are all songs in the heterogeneous network. There are $K$ communities generated by leveraging conventional methods. As in each community, the number of songs that $u$ listened before can be calculated, all communities are ranked by their contained number of listened songs in the descending order. Therefore $C_{u}^{k}$ means the community containing the $k_{th}$ most number of user $u$'s listened songs. $\rVert C_{u}^{k}\lVert$ is the number of nodes in this community. To make it easier to calculate, we define $\rVert C_{u}^{0}\lVert = 1$. $\varphi(s|u)$ is the number of times that user $u$ listens song $s$. $\mathbb{I}(s|u)$ is binary indicator $\in \{0,1\}$ to judge whether user $u$ listened the song before or not. 

This searching cost function depicts how much effort users take to retrieve all their listened songs by jumping between communities. For each user $u$, the  community ranking reveals how user $u$ favors to each community. The user $u$ starts to search from the most favoured community to the least favoured community in a descending sequence until all listened songs are retrieved. Formula \ref{eq:cost} defines a searching cost for all testing users jumping between communities. Community sizes of previous community and current community are considered during community jumping as larger community will take users more effort to find the listened songs. The searching cost also has a reciprocal relationship with the number of times users listened on songs because for more favored songs, the searching cost to retrieve them should be less. 
We calculate communities generated with/without ETUD with six classic conventional community detection algorithms (See Section 2 for algorithm description) and compare the searching cost of retrieving the top 5,10,20,50,100 listened songs for all testing users (songs are ranked by the number of listening times). The result is shown in Table \ref{tab:cost}.

  \begin{table}
        % \scriptsize
        \centering
%   \setlength{\abovecaptionskip}{-0.5cm}
% \setlength{\belowcaptionskip}{-0.cm}      
    %   \vspace{-3em} 
    \renewcommand{\tabcolsep}{1pt}
    % \hskip-2.8cm
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
       \textbf{Algorithm} &  \textbf{Category} & \textbf{Edge-type} & \textbf{ Comm. \#}   &\textbf{Cost@5} &\textbf{Cost@10}  &\textbf{Cost@20}   &\textbf{Cost@50}   &\textbf{Cost@100}  \\ \hline 
         \multirow{2}{*}{DeepWalk \cite{perozzi2014deepwalk}}  &  \multirow{2}{*}{embedding}    &  No  &100    &  197.29   &    420.01 & 897.37  &2309.50  &4450.39\\ 
           &      &  Yes   &  100 & \textbf{187.99}    &\textbf{402.51}    &\textbf{856.04}   &\textbf{2054.70}  &\textbf{4121.64} \\ \hline 
         \multirow{2}{*}{LINE \cite{tang2015line}}  &  \multirow{2}{*}{embedding}    &  No  &100    &   172.03 &   379.08  & 811.87  & 2106.40 & 4134.17\\ 
           &      &  Yes   & 100  &  \textbf{162.29}  & \textbf{371.29}    & \textbf{783.70}  & \textbf{2012.18} & \textbf{3922.18}\\ \hline 
         \multirow{2}{*}{node2vec \cite{grover2016node2vec}}  &  \multirow{2}{*}{embedding}    &  No  &   100 & 181.84  &  391.83 &849.79  & 2175.11 & 4132.87\\ 
           &      &  Yes   & 100  & \textbf{173.60}  & \textbf{390.29}    & \textbf{824.02}  & \textbf{2096.56} & \textbf{3984.89}\\ \hline 
        \multirow{2}{*}{Louvain \cite{blondel2008fast}}  &  \multirow{2}{*}{modularity}    &  No  & 12   & 577.40   &1275.62 & 2695.33  & 6925.05 & 12845.07\\ 
           &      &  Yes   & 38  & \textbf{533.19}   &  \textbf{1092.83} &  \textbf{2350.49} & \textbf{5963.32} &\textbf{10532.66} \\ \hline 
         \multirow{2}{*}{Infomap \cite{bohlin2014community}}  &  \multirow{2}{*}{random walk}    &  No  &  3705  &  850.09    & 1918.62   &  4022.01 & 10372.20 &19784.88 \\ 
           &      &  Yes   & 4507  &\textbf{682.42}   & \textbf{1571.91}  & \textbf{3358.09}  &\textbf{8494.20} &\textbf{15997.72} \\ \hline 
         \multirow{2}{*}{BigClam \cite{yang2013overlapping}}  &  \multirow{2}{*}{overlapping}    &  No  &   100 & 11.23 &    27.80 & 56.73  & 131.87& 270.42\\ 
           &      &  Yes   & 100  & \textbf{7.91}   &  \textbf{16.68}  & \textbf{39.36} & \textbf{105.74} & \textbf{183.10}\\ \hline 
       
         \end{tabular}
         \caption{Searching cost results comparison}
         \label{tab:cost}
         \vspace{-2em}
 \end{table} 
 Although different algorithms have different-scale searching costs and community number, all community results learned with ETUD require less searching cost than the communities without considering ETUD significantly. It means that learning ETUD via our model on heterogeneous network can reduce users' effort to search their favoured songs.
 
 
\subsection{Searching Accuracy within Community}

After exploring how well ETUD can help to reduce searching costs, we are also willing to see whether it also benefits music recommendation accuracy within communities. Ideally, the learned ETUD should have positive effect to group users and their favoured songs into the same community. In this task, for each testing user $u$, we select all songs in the same community as the user, and rank the songs based on their PageRank scores calculated during the training process. NDCG is still the evaluation metric used to evaluate how well the generated PageRank result matches user real listening history. The averaged NDCG score for all testing users is in Table \ref{tab:ranking}.
%Moreover, during the ETUD learning process, all nodes' PageRank scores are also calculated as the same time. Therefore, for the 50 users, we are willing to know whether musics in the same community with a user $u$ have a more similar ranking with the help of learned ETUD. As each user has a music listening history record in which all listened song $S$ is associated with listening time $g(S|u)$. And in the user's community, all songs are with PageRank score $p(S|u)$. We want to explore how well ETUDs can enhance the retrieval accuracy. In this paper, NDCG is used as the primary evaluation metric to quantify how well $p(S|u)$ matches $g(S|u)$. Six classic community detection models in three different categories are used to generate community partition for both non-ETUD network and ETUD network. Details of the community detection models are in the Section Related works. 
From the result, under all circumstances, NDCG scores with ETUD are significantly higher than scores without ETUD. It infers that by taking ETUD into account, it is more likely to group users and their favoured songs into the same community. %Therefore, when we recommend songs to users, we can first consider the songs within the same community as users instead of the whole network.

  \begin{table}
    % \scriptsize
    \centering
    %  \setlength{\abovecaptionskip}{-0.5cm}
    % \setlength{\belowcaptionskip}{-0.cm}
    %   \vspace{-3em} 
    \renewcommand{\tabcolsep}{2pt}
    
    \begin{tabular}{|c|c|c|c|c|c|} \hline
       \textbf{Algorithm} &  \textbf{Edge-type}    &\textbf{NDCG @5} &\textbf{NDCG@10}  &\textbf{NDCG@20}   &\textbf{NDCG@100}   \\ \hline 
         \multirow{2}{*}{DeepWalk}  &    No    & 0.6932  &  0.6974   &  0.6971  &  0.5741   \\ 
           &    Yes   &  \textbf{0.7529}  &  \textbf{0.7355} & \textbf{0.7162} & \textbf{0.5992}    \\ \hline 
         \multirow{2}{*}{LINE}  &     No &   0.4883 &0.3588    &  0.2530  &  0.1055   \\ 
           &   Yes   &\textbf{0.5153} & \textbf{0.4141}  & \textbf{0.3057} &  \textbf{0.1401} \\ \hline 
         \multirow{2}{*}{node2vec}  &   No   & 0.6995   &  0.7007 & 0.6967  & 0.5796  \\ 
           &  Yes    &  \textbf{0.7476}  & \textbf{0.7349}  &  \textbf{0.7206} &  \textbf{0.5924} \\ \hline 
        \multirow{2}{*}{Louvain}  &   No  &  0.6764  & 0.6742   &  0.6829  &  0.7168   \\ 
           &    Yes  & \textbf{0.7370}  & \textbf{0.7366} &  \textbf{0.7328} & \textbf{0.7328}    \\ \hline 
         \multirow{2}{*}{Infomap}  &    No   & 0.7020 & 0.6955 & 0.6974 & 0.7264  \\ 
           &   Yes   & \textbf{0.7548}  & \textbf{0.7430}  & \textbf{0.7332}  &  \textbf{0.6927}  \\ \hline 
         \multirow{2}{*}{BigClam}  &   No &  0.5963  &   0.5193 &  0.4524  &  0.2626  \\ 
           &  Yes    &  \textbf{0.6479} & \textbf{0.5793}  & \textbf{0.5022}  &  \textbf{0.2376}   \\ \hline 
       
         \end{tabular}
         \caption{Within-community music retrieval accuracy evaluation}
         \label{tab:ranking}
         \vspace{-4em}
 \end{table} 



==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/intro.tex <==
\section{Introduction}
 \vspace{-1em}
According to a new report released by Nielsen Music, on average, Americans now spend more than 32 hours a week listening to music\footnote{https://www.forbes.com/sites/hughmcintyre/2017/11/09/americans-are-spending-more-time-listening-to-music-than-ever-before}. Besides, with the boom of online music streaming services (MSS) in the recent years,   user behaviors on MSS (e.g. Pandora and Spotify) become various as well. How to conduct all types of behavior information from MSS to support music recommendation becomes a challenging task. As user behaviors on songs can naturally form a complex heterogeneous network (in Figure \ref{fig:sample}), community detection approaches can be a potential solution to solve this recommendation task by grouping relevant users and songs to the same community. Hence, developing more comprehensive and robust community detection models is in urgent need. In this paper, conventional methods refer to methods are originally designed for homogeneous community detection. Although some other works have addressed on heterogeneous networks, they are mostly task-driven approaches and not able to directly apply on musicrecommendation. In this study, in order to build up a bridge for conventional methods to be eligible on heterogeneous networks, we propose a genetic based method to learn the \textit{edge-type usefulness distribution} (ETUD) on heterogeneous networks in an evolutionary manner. Our model can highlight those edge-types  more important for music recommendation by assigning higher weights on them. After that, all edges are updated by multiplying related ETUD values on their original weights, which converts a heterogeneous network to a homogeneous one.
\vspace{-2em}
\begin{figure}[!htb]\centering
	\includegraphics[width=0.8\columnwidth]{img/sample.png}  
	\caption{An example of how ETUD influences the community structure in a heterogeneous music network }
	\label{fig:sample}
	 \vspace{-2em} 
 \end{figure} %\vspace{-2em}

%Most of the state-of-art community detection algorithms are developed for homogeneous networks and limited their potential for heterogeneous networks. Learning ETUD makes it possible to leverage those existing algorithms to detect the optimized community structure on a heterogeneous network. In this paper, a genetic based approach is proposed to optimize ETUD in an evolution manner. With the optimized ETUD, better community partition of the heterogeneous networks can be retrieved, which is beneficial to retrieve and recommend the most relevant products to users. Figure ~\ref{fig:sample} depicts an example about how ETUD influences community partition and therefore music recommendation for users.
Figure \ref{fig:sample} shows an example of how ETUD supports music recommendation  on a sample music network from community viewpoint. Figure ~\ref{fig:sample}(a) ignores the edge-types and treats the network as a homogeneous one. By leveraging a conventional community detection method (Louvain method \cite{blondel2008fast}), the whole music network is partitioned into two communities. while Figure \ref{fig:sample}(b) takes ETUD into account. The thickness of an  edge-type refer to its learned ETUD weight. Obviously the \emph{plays} edge-type is more important for music recommendation. After all edge weights are updated by multiplying related ETUD values, four communities are detected by leveraging the same community detection method. Comparing the two community detection results, it is clear to see that involving ETUD can be beneficial to group the user and his/her favored songs to the same community, which supports music recommendation to achieve better accuracy. 

%In order to evaluate the proposed method, we validate the new method on a large real-world music sharing network. We also propose a new evaluation metric, \textit{Community-based Searching Cost}, to tell the community structure usefulness in an information retrieval context (e.g., if the community information can assist users more efficiently access high-quality musics). 


 
The contribution of this paper is threefold:

\begin{itemize}
    \item First, a genetic based approach is used to learn ETUD on the heterogeneous networks in an evolutionary manner. It converts a heterogeneous network to a homogeneous one to enable conventional community detection methods on heterogeneous networks as well.
    \item Second, two evaluation tasks are proposed to validate the positive influence of ETUD on heterogeneous networks from searching cost and recommendation accuracy viewpoints. 
    \item  Third, extensive experiments applied on a music online streaming service dataset, Xiami Music, validate that our proposed model is feasible for music recommendation in real cases. 
\end{itemize}


%The paper is organized as following: Section 2 introduces related works on homogeneous \& heterogeneous community detection as well as music retrieval and recommendation; Section 3 explains our genetic based approach for ETUD optimization; Section 4 shows the experiment result on a real-world music network; Section 5 draws a conclusion and points out future work. 


==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/literature.tex <==
\section{Related works}
\textbf{Homogeneous Community Detection} Current studies follow four main trends \cite{gao2020community}: random walk, embedding, Modularity and overlapping community. node2vec \cite{grover2016node2vec}, DeepWalk \cite{perozzi2014deepwalk} and LINE \cite{tang2015line} are three representative models to learn node embeddings by maximizing the probability to reproduce the network structures. Louvain method \cite{blondel2008fast} designs an agglomerative framework to detect communities with largest Modularity score in an efficient manner.  Infomap \cite{bohlin2014community} assumes a random walker wanders on the network, and minimizes the cost to track the walker's path. Bigclam \cite{yang2013overlapping} formulates overlapping community detection problems into non-negative matrix factorization. \cite{gao2020detecting,ma2017document} leverage cross-domain information for sparse network community detection.

\textbf{Heterogeneous Community Detection} 
\cite{tang2012community} formally describe the heterogeneous community detection problem with a framework of four integration schemes. \cite{huang2018overlapping} aims at overlapping community detection on heterogeneous networks. \cite{comar2012simultaneous} decomposes the heterogeneous network to multiple simple networks. \cite{xie2014community} constructs user profiles from folksonomy systems and use the profiles as auxiliary information for user community detection. \cite{sun2013pathselclus} proposes to use metapath to control node communities with distinct semantics.


\textbf{Community-based Music Recommendation}
\cite{donaldson2007hybrid} considers both user behaviors on playlists and music content profile. \cite{bu2010music} constructs a hypergraph to model the multi-type objects in a music social community. \cite{guo2016feature} focuss on edge-type selection in the heterogeneous network to retain main semantic meanings and trim the network to a smaller scope. Derived from \cite{gao2017personalized}, \cite{gao2019efficient} proposes a generic algorithm for music recommendation guided by user information need.
% \textbf{[Community detection models]} Community detection is a traditional research topic and has been well addressed for years. Numerous studies design community detection models from various aspects such as random walk, embedding, modularity and overlapping communities. These models so far can really performs well to generate reliable communities on homogeneous networks. node2vec \cite{grover2016node2vec}, DeepWalk \cite{perozzi2014deepwalk} and LINE \cite{tang2015line} are three representative models to learn node embeddings by maximizing the probability to generate neighbour nodes for each node. And communities are calculated using the node embeddings. Different from embedding methods, by optimizing a well known community metric, modularity, Louvain method \cite{blondel2008fast} designs an agglomerative framework to learn the community structure in an efficient manner.  Infomap \cite{bohlin2014community} assumes a random walker wanders on the network, and minimizes the cost to track the walker's path. Bigclam \cite{yang2013overlapping} formulates community detection problems into non-negative matrix factorization
% and discovers overlapping community membership factors of nodes by maximum likelihood estimation. All those models are limited to solve community detection problem on homogeneous networks.% When the relationships between nodes are complex in the network, these models can't perform reliable community structures any more.
 
% \\ 
% \textbf{[Community detection in information retrieval]} Community structure can benefit information retrieval and recommendation accuracy by trimming searching scope, reducing searching cost and exploring node hidden relationships on networks. For instance, \cite{liu2005finding} investigated expert retrieval problem in an open-domain QA service by detecting communities within it.  \cite{cutting2017scatter} developed a Scatter/Gather model by considering community detection strategy on big document collections to accelerate the speed to browse and search documents.
% \cite{papadopoulos2012community} is a well known survey to broadly introduce  how community detection methods effecting in the context of real-world web mining and information retrieval scenarios.

==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/method.tex <==
\section{Method}
 \vspace{-1em}
In this section, a genetic approach is proposed here to learn the \textit{edge-type usefulness distribution} (ETUD). ETUD is the weights for all edge-types to represent their usefulness towards the network. After each edge's weight is updated by multiplying related ETUD score to its original value according to its edge-type, a heterogeneous network is converted to a homogeneous one. Figure \ref{fig:pipeline} shows the proposed method in detail.  

\vspace{-1em} 
\begin{figure}[!htb]\centering
	\includegraphics[width=0.8\columnwidth]{img/approach.png}  
	\caption{Genetic approach to learn ETUD in an evolutionary manner}
	\label{fig:pipeline}
	 \vspace{-3em} 
 \end{figure} %\vspace{-2em}

\subsection{ETUD Initialization}  
In our genetic approach, the whole process simulates biological evolution process. We define a \emph{chromosome} to represent a possible ETUD result. A \emph{chromosome} is constructed by a set of \emph{gene}s ,where each \emph{gene} refers to an edge-type respectively. The value stores in each \emph{gene} represents the usefulness score of a particular edge-type. A \emph{chromosome} is initialized by randomly assigning value $\in [0,1]$ to each of its \emph{gene} in the beginning. In total, $P$ \emph{chromosome}s are randomly initialized for further evolution process.

%Same as most of optimization problems, the first initialization step assigns ETUD values with random start. To ensure all ETUD values under probability distribution, each randomized edge-type $e_{i}$ in ETUD can be set a value within a restricted boundary $e_{i} \in [0,1]$. In the end, a set of $p$ random generated ETUDs are initialized.

\subsection{ETUD Assessment and Selection} 
Given $P$ \emph{chromosome}s, a fitness function   needs to be set up as a criteria to evaluate each \emph{chromosome}'s performance for music recommendation. The best ETUD should be able to best reproduce users' listening preference. In other words, we should find an ETUD that maximizes the similarity between songs' ranking list generated under this ETUD  and user real preference on songs, which is described in Formula \ref{eq:objective}:  



%help to generate all songs $S$ ranking list $Ranking(S|w,u)$ to best match the user $u$'s listening preference  $g(S|u)$ (e.g., songs listened by the user $u$). And the objective function we need to maximize should be:

\begin{equation}
  \argmax_\textit{w} \sum_{u \in U} sim (g(S|u),p(S|u;w))
  \label{eq:objective}
\end{equation}

$w$ is the  \emph{chromosome} we aim to retrieve, $U$ is the set of all users and $S$ is the set of all songs in the music network.  $g(S|u)$ is the real listening preference of user $u \in U$; $p(S|u;w)$ is all songs ranking list we estimated for user $u$ given the ETUD $w$. Function $sim(\cdot)$ measures the similarity between the two ranking lists. It is hard to leverage stochastic gradient decent on Formula \ref{eq:objective} directly as the differential of $p(S|u;w)$ may be too complex to compute. Genetic approach offers an evolution process to solve this challenge instead. As there are in total $P$ \emph{chromosome}s representing possible ETUD results, we can evaluate each \emph{chromosome} and select better ones to bring offspring \emph{chromosome}s. We call a cycle of selecting \emph{chromosome}s and breeding new offspring \emph{chromosome}s as a \emph{generation}. The whole evolution process will keep running until the fittest  \emph{chromosome} in each \emph{generation} no longer changes. Derived from Formula \ref{eq:objective}, In this paper, each \emph{chromosome}'s fitness value can be calculated as:
\begin{equation}
\textit{$f(w)$} = \frac{exp(\sum_{u \in U} sim( g(S|u),p(S|u;w))}{\sum_{p \in P}exp(\sum_{u \in U} sim( g(S|u),p(S|u;p))} 
\label{eq:fitness}
\end{equation} 

Personalized PageRank algorithm \cite{kloumann2017block} is utilized to represent user $u$ listening preference $p(S|u;w)$. Based on empirical study and common sense that users may only pay attention to the top recommended songs, NDCG@10 \cite{wang2013theoretical} is chosen as the similarity judging function $sim(\cdot,\cdot)$ in this paper. NDCG@10 is an evaluation metric to judge how well the estimated ranking list $p(S|u;w)$ matches the user $u$'s real listening preference $g(S|u)$ and is more sensitive to top ranked results. To represent the fitness score of \emph{chromosome} $w$, we calculate the similarity scores among all users and normalize it via a Softmax function on all \emph{chromosome}s.

In genetic approach, \emph{chromosome}s with higher fitness score should have higher chance to be preserved for the next-round evolution. Hence, we use bootstrap sampling strategy (random sampling with replicates) to randomly sample $P$ \emph{chromosome}s based on their fitness scores. This sampling strategy has two advantages: First, there are always $P$ \emph{chromosome}s in each generation, which ensures a stable evolution process; Second, \emph{chromosome}s with higher fitness scores are more likely to be preserved, so that the best ETUD result is more likely to be found after running a number of \emph{generation}s. 
% To accelerate computation efficiency, a MapReduce framework is utilized to enable genetic evolution parallelization. After a set of ETUD candidates are initialized, they are randomly split into $M$ groups for further parallel computing in the ``Splitter'' process. After that, $M$ chained mappers calculate all fitness scores in each group and project them back to related ETUD candidates. In a``Selection'' process, ETUD candidates are selected with a probability equal to their fitness scores in each individual group. And in the end the framework applies ``Reducer'' in cross-over process to generate new ETUD candidates  and mutation process via the chained Mappers to execute mutations on newly generated ETUD candidates individually. By leveraging this parallel approach, each group can be calculated separately and simultaneously in the evolution process. 


\subsection{ETUD Transformation} 

The initialized \& selected \emph{chromosome}s can not fully cover the whole possible ETUD results. Hence, there is a need to search the whole ETUD result space and find out the best one. To achieve this in an efficient manner, two transformation strategies including  Cross-over and Mutation are applied. These two strategies help to generate new \emph{chromosome}s from the the original selected \emph{chromosome}s, which achieves the \emph{chromosome} evolution. 

Specifically, In Cross-over step, all selected \emph{chromosome}s are grouped into pairs first, and the Cross-over transformation will be applied within pairs. Given two \emph{chromosome}s in the same pair, which are denoted as $w_1$ and $w_2$.  In this step, $w_1$ and $w_2$ exchange values stored in partial of their genes to create two offspring \emph{chromosome}s. $w_{1k}$ refers to the edge-type usefulness weight stored in the $k_{th}$ gene of $w_1$. The whole process is showed as: 
% \begin{align} 
% w_{1i} = \alpha* w_{1i}+(1-\alpha)* w_{2i} \nonumber \\ 
% w_{2i} = \alpha* w_{2i}+(1-\alpha)* w_{1i}
% \end{align}
\begin{equation}
w_{ij}^{*} = 
(\frac{w_{ij}}{ w_{1j}+ w_{2j}})^{p_j}w_{ij}^{(1-p_j)}
\label{eq:transform}
\end{equation}
\begin{eqnarray}\text{$p_j$}=
\begin{cases}
\text{$1$}, & r_j \ge t_c\cr 
\text{$0$}, &  r_j < t_c
\end{cases}
\label{eq:binary}
\end{eqnarray}
where $i \in \{1,2\}$ refers to the index of the two newly generated \emph{chromosome}s. $w_{ij}$ is the value of the $j_{th}$ gene in $w_{i}$. $p_j$ is an binary indicator to decide whether the cross-over step occurs on the $j_{th}$ gene or not. The value of $p_j$ is controlled by a randomly generated variable $r_j \in [0,1]$ and a pre-defined threshold $t_c \in [0,1]$. 

Unlike the Cross-over step to generate new offspring \emph{chromosome}s via the interactions between two original \emph{chromosome}s, Mutation step allows a \emph{chromosome} to generate a new offspring \emph{chromosome} within itself. For \emph{chromosome} $w_{1}$, instead of exchanging values of genes with another \emph{chromosome} $w_{2}$, it exchanges its genes' value with a random variable $\mathcal{X}$ randomly drew from normal distribution $\mathcal{X} \sim \mathcal{N}(0,1)$. And the gene values of new \emph{chromosome} is still calculated via Formula \ref{eq:transform} and \ref{eq:binary} with another pre-defined threshold $t_m \in [0,1]$.
% \begin{equation}
% W_{ij}^{*} =  \delta
% (\frac{exp(W_{ij})}{ exp(W_{ij})+ exp(r)}) 
% \end{equation}

% where $r \sim \mathbb{N}(0,1)$. Both transformation steps use a softmax function to normalize the results within the range \{0,1\}.

\subsection{ETUD Finalization}

The whole evoluntion process will keep running for \emph{generation}s until the best \emph{chromosome} no longer changes for $\mathbb{N}$ generations. And the \emph{chromosome} with largest fitness value in the last \emph{generation} will be the returned ETUD.

However, there is still an edge-type dependency issue remained. One example viewed in Figure \ref{fig:sample} is that edge-type \emph{performIn} and edge-type \emph{plays} are independent so that their weights are not comparable. To address this, we define: 

\begin{Definition}
Two edge-types are dependent only if they share either same start-node type or same end-node type. And only weights of dependent edge-types are comparable.
\label{def:dependency}
\end{Definition}


Following Definition \ref{def:dependency}, all edge-types are grouped into several independent sets first ( In Figure \ref{fig:sample}, the edge-type sets are \{\emph{performsIn}, \emph{includes}\} and \{\emph{plays}, \emph{bookmarks}\}). After that, ETUD weights of edge-types in the same set are normalized via the formula:
\begin{equation}
\textit{$ew_i^{*}$} = \frac{ew_{i}}{\sum_{S(e_{i}) = S(e_{j})}ew_{j}} 
\end{equation} 

$e_{i}$ refers to the $i_{th}$ edge-type; $ew_{i}$ refers to the returned ETUD weight of edge-type $e_{i}$; $S(e_{i})$ is the edge-type set which $e_{i}$ belongs to. And the normalized $ew_i^{*}$ is regarded as the final edge-type usefulness weight of $e_{i}$.

==> Improving Community Detection Performance in Heterogeneous Music Network by Learning Edge-type Usefulness Distribution/content/test.tex <==
  \begin{table*}
        % \scriptsize
        \centering
    %   \vspace{-3em} 
    % \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|} \hline
        \multirow{2}{*}{\textbf{algorithm}} &  \multirow{2}{*}{\textbf{category}} & \multicolumn{2}{c}{\textbf{non edge-type learning}} & \multicolumn{2}{|c|}{\textbf{with edge-type learning $\alpha$ = 0.9}}  \\  
          &   & \textbf{cluster number}   &\textbf{searching cost} & \textbf{cluster number}   &\textbf{searching cost}         \\ \hline 
         deepWalk  &  embedding    &  100  &  12749.95  &  100  &  11974.05    \\ 
         LINE  &  embedding  &  100  &   9104.49 & 100   &  8889.81\\ 
         node2vec    & embedding  &  100 &   13719.31   & 100   &  11204.64\\
         Louvain  &  modularity   & 38   &  194778.93  &  12  &  20439.72     \\ 
         Infomap  & random walk   &  3705  &   2.19E9 &  4507  & 1.46E9   \\ 
         BigClam    & overlapping  & 100  & 960.20   &  100  &    440.86\\
         \hline  
         \end{tabular}
         \caption{Search cost result comparison, search time cost is standardized}
         \label{tab:multiclass}
 \end{table*} 
 
 \section{Method}

\subsection{Candidate initialization}
\subsection{Edge-type weight evaluation}
\subsection{}
\subsection{}

In order to solve this task, we propose a genetic algorithm approach whose core idea is derived from a biological involution process with four main steps: \textbf{Initialization},  \textbf{Selection},  \textbf{Cross-over}, and \textbf{Mutation}. Within genetic algorithm, a candidate result is called a `chromosome` which is constructed by a set of `genes`. And a set of candidate results  are initialized  as the first `generation`. In each iteration, the previous generation is processed through the four steps to generate an optimized `offspring` as the next generation. The iterative process will terminate until it reaches to an optimal case. Specifically, in our graph simplification approach, each edge type is regarded as a `gene` associated with weight, which means a `chromosome` can be regarded as a weight distribution of all edge types. If an edge type has a weight of 0, it means that this edge type is removed from the graph.   %Therefore, a chromosome can represent a potential edge type combination with weight, which can also be regarded as a solution of graph simplification. 
%Within genetic algorithm model, there are five sequential steps including initialization, fitness score calculation, selection, crossover and mutation. 

Specifically, in \textbf{Initialization} step, a `chromosomes` is  initialized by randomly assigning weights on its related `genes` (edge types). $P$ initialized `chromosomes` are generated in this way as the first generation where $P$ is the given size of a `chromosome` generation. Then, in \textbf{Selection} step, calculated by a pre-defined fitness function, each `chromosome` is evaluated with a fitness score where a larger fitness score implicates better a candidate result of graph simplification. Afterwards,  $P$ chromosomes are selected with duplicates based on fitness score and formed into pairs by the selection sequence. In \textbf{Cross-over} step, each pair of chromosomes have a certain probability to exchange partial genes so as to generate `offsprings`. Moreover, in \textbf{Mutation} step, each chromosome also has a small change to mutate partial genes within itself, which can also generate new `offsprings`. The whole process will repeat iteratively until the chromosome with largest fitness score stays stable. The `chromosome` with largest fitness score is returned as the final edge type weight distribution. 

%In genetic algorithm, a better fitness function can both accelerate the converging speed and generate better edge type weights for graph simplification. 
To evaluate the fitness of each `chromosome`, we involve an external $K$ users' listening history dataset as pseudo ground truth to represent users' listening preference. We assume a better edge-type weight distribution can better reproduce users' listening preference. Hence, in our model, the fitness score of `chromosome` $i$ is calculated as:

\begin{equation}
\textit{$f(ch_{i})$} = \frac{exp(\mathbb{E}_{k \in K} \Gamma(\mathnoraml{p}(k), \mathnoraml{g}(k)| ch_{i}))}{\sum_{p=1}^{P}exp(\mathbb{E}_{k \in K} \Gamma(\mathnoraml{p}(k), \mathnoraml{g}(k) | ch_{p}))} 
\end{equation} 

$p(k)$ is the PageRank ranking result of the songs listened by the $k$th user in the heterogeneous graph with edge type weight distribution $ch_{i}$; $g(k)$ is the songs listened by $k$th user's and ranked by the number of listening times. $\Gamma$ function is an evaluation function to judge how well the generated PageRank ranking list $p(k)$ matches the $k$th user's listening preference $g(k)$. It can be any IR related evaluation metrics such as precision, recall, NDCG, MAP, etc. In our approach, we decide to use Precision@10 as the evaluation criteria because users only focus on the top recommended songs usually. We calculate the expectation of precision results on all K users and apply a Softmax functions to normalize the fitness score of each `chromosome`.  %the real ranking list of node i while $PR(n_{i}$ is the Page Rank score ranking list of node i in the graph. We calculate the average of all K nodes' pairwised ranking precision score between Page Rank score ranking list and true ranking list, and regard the average precision score as \textit{$ch$}'s fitness score. 

%Hereby, an two step approach based on genetic algorithm is applied on the heterogeneous graph first to find the best edge type combination for our recommendation task. It includes edge weight initialization step and edge selection step. 

%To simplify a graph, calculating each edge type's weight via genetic algorithm and remaining edge types with high weight is an option.  %Therefore, the edge weight initialization step uses genetic algorithm to find the best edge type weight distribution so as to best match Pagerank ranking list with real data ranking list. In this step, a chromosome refers to a potential edge type weight distribution. After taking genetic algorithm steps iteratively, the best chromosome can be found until the whole process converges. 
Although genetic algorithm offers a strong theoretical foundation to solve graph simplification problem, two challenges are still waiting to be solved. First,  some edge types are independent with each other i.e. two edge types have both different start-node types and end-node types. To retrieve top $N$ edge types, it doesn't make sense to simply return the top $N$ edge types with highest weight value because weight values are incomparable if the two related edge types are independent. For instance, in a music graph, `listening` edge type between user and song is independent with `publish` relationship between artist and album. A higher weight of `listening` edge type does not mean a user-song relationship is more important than the relationship between an artist and the related album. Second, in our genetic approach, for each edge type weight distribution (chromosome), we have to run PageRank each time, it is time consuming when dealing with huge graphs. To tackle with the first challenge, we propose two separate genetic approaches to remove edge type dependency influence and find out the best $N$ edge types of the heterogeneous graph. And a MapReduce framework is applied to run the whole genetic process in parallel so that to reduce overall running time.% To remove the dependency influence on graph simplification, we propose a secondary genetic algorithm to find out best graph schema based on the edge-type weight combination result retrieved from the previous step.

In the first genetic approach, we ignore the dependency issue first and retrieve an edge type weight distribution $\{w_{1},w_{2},...,w_{t}\}$ for $t$ types of edges based on the genetic algorithm framework introduced in previous paragraphs. 

After that, we define two edge types are dependent if they share the same kind of either start node or end node. Follow this, all edge types are grouped into $m$ independent edge type sets $\{S_{1},S_{2},...,S_{m}\}$.%as $\{\{e_{1}, e_{2}, ..., e_{|m_{1}|}\}, \{e_{|m_{1}|+1}, e_{|m_{1}|+2}, ..., e_{|m_{1}|+|m_{2}|}\}, ... , \{e_{t-|m_{m}|+1}, e_{t-|m_{m}|+2}, ..., e_{t}\}\}$. 
We also normalize edge type weights in each independent sets following the formula:
\begin{equation}
\textit{$w_i^{*}$} = \frac{w_{i}}{\sum_{S(e_{i}) = S(e_{j})}w_{j}} 
\end{equation} 

%Second, within each independent edge set, edge-type weights are normalized to a probability distribution.

The second genetic approach is proposed based on the independent edge type sets and normalized edge type weights. Different from the first genetic approach, a `gene` here stores two values: a binary value $B$ to decide whether its related edge type is removed or kept and the normalized edge type weight calculated previously. 

In order to choose top $N$ edge types, for a `chromosome`,$N$ genes are with $B = 1$ and the rest $t-N$ genes have $B = 0$. binary values $B$ are exchanged in the Cross-over step, and the total number of genes with $B =1$ should be $N$ after the Mutation step, which means that each time a gene's binary value changes from 0 to 1, another gene should be randomly selected and its binary value changes from 1 to 0. When we calculate fitness score for a `chromosome`, only edge types (genes) with $B = 1$ are remained and their associated normalized weights $w$ are used to generate the PageRank ranking list $p(K)$ for all $K$ users. 

%The first two steps are preparations for the next secondary genetic algorithm step. Different from the previous genetic algorithm to generate edge type weight combination, a gene of current genetic algorithms refer to a type of selected edge, and its value is the edge-type weight calculated by the previous genetic algorithm. Therefore, a chromosome here refers to a combination of selected edge types. The number of genes refers to the number of edge types we want to choose.

To reach global optima faster, the initialization step of the second genetic algorithm uses a two-step sampling strategy including an edge type set selection process and an edge type selection process. 
 
% \[ \text{$P(S_{i})$} =
%   \begin{cases}
%   \frac{1}{M} , &   \text{$S_{i} \subseteq$ S}\\  0 , & \text{otherwise}\\
   
%   \end{cases}
% \]
% \begin{equation*}
% X \sim \mathcal{D}(S_{x})\, 
% \end{equation*}

First, one edge type set is randomly picked up from all independent edge-type sets following a uniform distribution. After a set $S_{1}$ is picked up, an edge type $e_{1}$ is selected based on its normalized edge-type weight. %This sampling process will continue unless  distinct edge types are selected.

%The rest of the steps are the same as previous genetic algorithms, including fitness function, selection, crossover, and mutation steps, which means initialized chromosomes are selected as pairs, processed via crossover and mutation steps, and, 

In the end, the `chromosome` with highest fitness score is returned as the final edge type selection result. And edge types with $B = 1$ are the selected top $N$ edge types which are remained in the heterogeneous graph. %salient edge-type combination which can best represent the entire heterogeneous graph. 

\begin{equation}
    Cost(u, S) = \sum_{s \in S}\mathbb{I}(G(u),G(s))\frac{C(u)*C(s)}{D(s|u)*\mu(\mathcal{N},\mathcal{C})^{2}} 
\end{equation}

C(u) and C(s) means the cluster size of user u and song s. $\mathcal{N}$ is the number of nodes in the graph, $\mathcal{C}$ is the number of communities. $\mu(\mathcal{N},\mathcal{C})$ is the average cluster size. D(s|u) is the preference degree of song s towards user u. $\mathbb{I}(u,s)$ is a judging function where:

\begin{equation}
  \mathbb{I}(G(u),G(s)) =
  \begin{cases}
    \alpha,       & \quad G(s) =  G(u)\\ 
    1-\alpha,  & \quad G(s) \neq  G(u)\\
  \end{cases}
  \label{eq:relu}
\end{equation}

$\alpha$ is from 0 to 1. G(s) refers to the community of s. 



==> content/copy.tex <==
\section{Results}

  \begin{table*}
        % \scriptsize
        \centering
    %   \vspace{-3em} 
    % \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|} \hline
        \multirow{2}{*}{\textbf{algorithm}} &  \multirow{2}{*}{\textbf{category}} & \multicolumn{2}{c}{\textbf{non edge-type learning}} & \multicolumn{2}{|c|}{\textbf{with edge-type learning $\alpha$ = 0.7}}  \\  
          &   & \textbf{cluster number}   &\textbf{searching cost} & \textbf{cluster number}   &\textbf{searching cost}         \\ \hline 
         deepWalk  &  embedding    &  100  &   3.6158   &  100  &  3.3958    \\ 
         LINE  &  embedding  &  100  &  2.5820    & 100   & 2.5211 \\ 
         node2vec    & embedding  &  100 &   3.8907   & 100   &  3.1776\\
         Louvain  &  modularity   & 12   &  3.8254   &  38  &    4.0254  \\ 
         Infomap  & random walk   &  3705  &   4.5357 &  4507  & 2.0513   \\ 
         BigClam    & overlapping  & 100  & 6.8448   &  100  &    4.8465\\
         \hline  
         \end{tabular}
         \caption{Search cost result comparison, search time cost is standardized}
         \label{tab:multiclass}
 \end{table*} 
 
 
 
 
 \begin{equation}
    Cost(u, S) = \sum_{s \in S}\mathbb{I}(G(u),G(s))\frac{C(u)*C(s)}{D(s|u)*\mu(\mathcal{N},\mathcal{C})^{2}} 
\end{equation}

C(u) and C(s) means the cluster size of user u and song s. $\mathcal{N}$ is the number of nodes in the graph, $\mathcal{C}$ is the number of communities. $\mu(\mathcal{N},\mathcal{C})$ is the average cluster size. D(s|u) is the preference degree of song s towards user u. $\mathbb{I}(u,s)$ is a judging function where:

\begin{equation}
  \mathbb{I}(G(u),G(s)) =
  \begin{cases}
    \alpha,       & \quad G(s) =  G(u)\\ 
    1-\alpha,  & \quad G(s) \neq  G(u)\\
  \end{cases}
  \label{eq:relu}
\end{equation}

$\alpha$ is from 0 to 1. G(s) refers to the community of s. 



  \begin{table*}
        % \scriptsize
        \centering
    %   \vspace{-3em} 
    % \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
       \textbf{algorithm} &  \textbf{category} & \textbf{edge-type weight} & \textbf{cluster number}   &\textbf{cost@5} &\textbf{cost@10}  &\textbf{cost@20}   &\textbf{cost@50}   &\textbf{cost@100}  \\ \hline 
         \multirow{2}{*}{DeepWalk}  &  \multirow{2}{*}{embedding}    &  No  &100    & 122.97   &   279.38 & 618.69  & 1562.37&3108.52\\ 
           &      &  Yes ($\alpha = 0.1$)  &  100 & 120.59   & 264.00   & 592.22  &1498.92 &2979.50\\ \hline 
         \multirow{2}{*}{LINE}  &  \multirow{2}{*}{embedding}    &  No  &100    &  95.62  &  213.37  & 456.83  & 1188.40&2298.26\\ 
           &      &  Yes ($\alpha = 0.1$)  & 100  & 91.45   &  211.23  & 444.95  & 1148.25&2227.35\\ \hline 
         \multirow{2}{*}{node2vec}  &  \multirow{2}{*}{embedding}    &  No  &   100 & 135.95   & 303.41   & 667.21  & 1698.62&3337.78\\ 
           &      &  Yes ($\alpha = 0.1$)  & 100  &  108.77  &  246.79  & 549.21  & 1385.76&2750.14\\ \hline 
        \multirow{2}{*}{Louvain}  &  \multirow{2}{*}{modularity}    &  No  & 38   &  2039.15  &  4240.29  & 9228.21  & 24045.29&47382.69\\ 
           &      &  Yes ($\alpha = 0.1$)  & 12  &  211.40  & 419.63   & 912.34  &2374.08 &4658.48\\ \hline 
         \multirow{2}{*}{Infomap}  &  \multirow{2}{*}{random walk}    &  No  &  3705  &  2.43E7   &   5.31E7 & 1.11E8  & 2.82E8&5.45E8\\ 
           &      &  Yes ($\alpha = 0.1$)  & 4507  & 1.68E7   &  3.52E7  & 7.25E7  &1.80E8 &3.51E8\\ \hline 
         \multirow{2}{*}{BigClam}  &  \multirow{2}{*}{overlapping}    &  No  &   100 &  4.47  &  19.80  & 55.59  &116.67 &193.59\\ 
           &      &  Yes ($\alpha = 0.1$)  & 100  & 3.00   &  8.77  &  19.17 & 41.52&82.80\\ \hline 
       
         \end{tabular}
         \caption{Search cost result comparison, search time cost is standardized}
         \label{tab:cost}
 \end{table*} 
 \begin{figure}
\subfloat[DeepWalk]{\includegraphics[width = 1.2in]{deepwalk.png}}
\subfloat[LINE]{\includegraphics[width = 1.2in]{line.png}}
\subfloat[node2vec]{\includegraphics[width = 1.2in]{node2vec.png}}\
\subfloat[Louvain]{\includegraphics[width = 1.2in]{louvain.png}} 
\subfloat[Infomap]{\includegraphics[width = 1.2in]{infomap.png}}
\subfloat[BigClam]{\includegraphics[width = 1.2in]{bigclam.png}} 
\caption{Tuning $\alpha$ of searching cost in six community detection algorithsm}
 \vspace{-1em}
 \label{fig:tune}
\end{figure} 
 

==> content/data_copy.tex <==
\section{Data Preparation}

To test the effectiveness of the proposed approach, we collected a large dataset from an online music streaming system. Like many online music streaming services, the system allows users to play music on-demand, create and share playlists, bookmark and comment for their favorite artists and songs. In addition to bibliographical music metadata (artist, album, song, genre), we also collected the listening history of a large number of users, and other types of interaction these users performed on the service (the playlists they've created on the service, what artists/songs/albums they have bookmarked or commented on, etc.). The collected dataset contains 56,055 artists, 43,086 albums, 1,233,651 songs, 633 genres, 677,275 users, 305,916 playlists, and 15,879,347 relations between them. We randomly selected 500 users who have at least 50 songs in their listening history for test purpose. We use 60\% of the songs in their listening history to train the personal navigation profile, and the other 40\% are used for evaluation. We use another 500 users selected with the same criteria for global navigation profile training.

The heterogeneous music schema contains 6 types of nodes, and 32 types of edges (a relation and its reverse relation are considered belonging to two different edge types). We used a relatively simple heterogeneous graph with 6 types of edges for parameter tuning. The six edge types are artist-performsIn-song, album-includes-song, user-plays-song, and their reverse types.

In music recommendation domain, play count is generally considered a type of implicit feedback. Unlike explicit rating, the number of times a song is played is collected passively and contains a lot of noise (e.g. the user forgets to pause the player when her listening is interrupted) and does not accurately reflect the degree of preference from the user. It is generally agreed that the user listening to a song indicates the song appeals to her in some way, and the majority of the remaining songs in the catalog are less so. Thus, we use play counts as a binary indicator of whether the user has interest in a song, in all our experiments reported in this paper.
\begin{figure}[!htb]\centering
	\includegraphics[width=0.9\columnwidth]{paper/graphScheme.jpg}  
	\caption{Graph schema.}
	\label{fig:graph}
 \end{figure} %\vspace{-2em}



==> content/test.tex <==
  \begin{table*}
        % \scriptsize
        \centering
    %   \vspace{-3em} 
    % \renewcommand{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|} \hline
        \multirow{2}{*}{\textbf{algorithm}} &  \multirow{2}{*}{\textbf{category}} & \multicolumn{2}{c}{\textbf{non edge-type learning}} & \multicolumn{2}{|c|}{\textbf{with edge-type learning $\alpha$ = 0.9}}  \\  
          &   & \textbf{cluster number}   &\textbf{searching cost} & \textbf{cluster number}   &\textbf{searching cost}         \\ \hline 
         deepWalk  &  embedding    &  100  &  12749.95  &  100  &  11974.05    \\ 
         LINE  &  embedding  &  100  &   9104.49 & 100   &  8889.81\\ 
         node2vec    & embedding  &  100 &   13719.31   & 100   &  11204.64\\
         Louvain  &  modularity   & 38   &  194778.93  &  12  &  20439.72     \\ 
         Infomap  & random walk   &  3705  &   2.19E9 &  4507  & 1.46E9   \\ 
         BigClam    & overlapping  & 100  & 960.20   &  100  &    440.86\\
         \hline  
         \end{tabular}
         \caption{Search cost result comparison, search time cost is standardized}
         \label{tab:multiclass}
 \end{table*} 
 
 \section{Method}

\subsection{Candidate initialization}
\subsection{Edge-type weight evaluation}
\subsection{}
\subsection{}

In order to solve this task, we propose a genetic algorithm approach whose core idea is derived from a biological involution process with four main steps: \textbf{Initialization},  \textbf{Selection},  \textbf{Cross-over}, and \textbf{Mutation}. Within genetic algorithm, a candidate result is called a `chromosome` which is constructed by a set of `genes`. And a set of candidate results  are initialized  as the first `generation`. In each iteration, the previous generation is processed through the four steps to generate an optimized `offspring` as the next generation. The iterative process will terminate until it reaches to an optimal case. Specifically, in our graph simplification approach, each edge type is regarded as a `gene` associated with weight, which means a `chromosome` can be regarded as a weight distribution of all edge types. If an edge type has a weight of 0, it means that this edge type is removed from the graph.   %Therefore, a chromosome can represent a potential edge type combination with weight, which can also be regarded as a solution of graph simplification. 
%Within genetic algorithm model, there are five sequential steps including initialization, fitness score calculation, selection, crossover and mutation. 

Specifically, in \textbf{Initialization} step, a `chromosomes` is  initialized by randomly assigning weights on its related `genes` (edge types). $P$ initialized `chromosomes` are generated in this way as the first generation where $P$ is the given size of a `chromosome` generation. Then, in \textbf{Selection} step, calculated by a pre-defined fitness function, each `chromosome` is evaluated with a fitness score where a larger fitness score implicates better a candidate result of graph simplification. Afterwards,  $P$ chromosomes are selected with duplicates based on fitness score and formed into pairs by the selection sequence. In \textbf{Cross-over} step, each pair of chromosomes have a certain probability to exchange partial genes so as to generate `offsprings`. Moreover, in \textbf{Mutation} step, each chromosome also has a small change to mutate partial genes within itself, which can also generate new `offsprings`. The whole process will repeat iteratively until the chromosome with largest fitness score stays stable. The `chromosome` with largest fitness score is returned as the final edge type weight distribution. 

%In genetic algorithm, a better fitness function can both accelerate the converging speed and generate better edge type weights for graph simplification. 
To evaluate the fitness of each `chromosome`, we involve an external $K$ users' listening history dataset as pseudo ground truth to represent users' listening preference. We assume a better edge-type weight distribution can better reproduce users' listening preference. Hence, in our model, the fitness score of `chromosome` $i$ is calculated as:

\begin{equation}
\textit{$f(ch_{i})$} = \frac{exp(\mathbb{E}_{k \in K} \Gamma(\mathnoraml{p}(k), \mathnoraml{g}(k)| ch_{i}))}{\sum_{p=1}^{P}exp(\mathbb{E}_{k \in K} \Gamma(\mathnoraml{p}(k), \mathnoraml{g}(k) | ch_{p}))} 
\end{equation} 

$p(k)$ is the PageRank ranking result of the songs listened by the $k$th user in the heterogeneous graph with edge type weight distribution $ch_{i}$; $g(k)$ is the songs listened by $k$th user's and ranked by the number of listening times. $\Gamma$ function is an evaluation function to judge how well the generated PageRank ranking list $p(k)$ matches the $k$th user's listening preference $g(k)$. It can be any IR related evaluation metrics such as precision, recall, NDCG, MAP, etc. In our approach, we decide to use Precision@10 as the evaluation criteria because users only focus on the top recommended songs usually. We calculate the expectation of precision results on all K users and apply a Softmax functions to normalize the fitness score of each `chromosome`.  %the real ranking list of node i while $PR(n_{i}$ is the Page Rank score ranking list of node i in the graph. We calculate the average of all K nodes' pairwised ranking precision score between Page Rank score ranking list and true ranking list, and regard the average precision score as \textit{$ch$}'s fitness score. 

%Hereby, an two step approach based on genetic algorithm is applied on the heterogeneous graph first to find the best edge type combination for our recommendation task. It includes edge weight initialization step and edge selection step. 

%To simplify a graph, calculating each edge type's weight via genetic algorithm and remaining edge types with high weight is an option.  %Therefore, the edge weight initialization step uses genetic algorithm to find the best edge type weight distribution so as to best match Pagerank ranking list with real data ranking list. In this step, a chromosome refers to a potential edge type weight distribution. After taking genetic algorithm steps iteratively, the best chromosome can be found until the whole process converges. 
Although genetic algorithm offers a strong theoretical foundation to solve graph simplification problem, two challenges are still waiting to be solved. First,  some edge types are independent with each other i.e. two edge types have both different start-node types and end-node types. To retrieve top $N$ edge types, it doesn't make sense to simply return the top $N$ edge types with highest weight value because weight values are incomparable if the two related edge types are independent. For instance, in a music graph, `listening` edge type between user and song is independent with `publish` relationship between artist and album. A higher weight of `listening` edge type does not mean a user-song relationship is more important than the relationship between an artist and the related album. Second, in our genetic approach, for each edge type weight distribution (chromosome), we have to run PageRank each time, it is time consuming when dealing with huge graphs. To tackle with the first challenge, we propose two separate genetic approaches to remove edge type dependency influence and find out the best $N$ edge types of the heterogeneous graph. And a MapReduce framework is applied to run the whole genetic process in parallel so that to reduce overall running time.% To remove the dependency influence on graph simplification, we propose a secondary genetic algorithm to find out best graph schema based on the edge-type weight combination result retrieved from the previous step.

In the first genetic approach, we ignore the dependency issue first and retrieve an edge type weight distribution $\{w_{1},w_{2},...,w_{t}\}$ for $t$ types of edges based on the genetic algorithm framework introduced in previous paragraphs. 

After that, we define two edge types are dependent if they share the same kind of either start node or end node. Follow this, all edge types are grouped into $m$ independent edge type sets $\{S_{1},S_{2},...,S_{m}\}$.%as $\{\{e_{1}, e_{2}, ..., e_{|m_{1}|}\}, \{e_{|m_{1}|+1}, e_{|m_{1}|+2}, ..., e_{|m_{1}|+|m_{2}|}\}, ... , \{e_{t-|m_{m}|+1}, e_{t-|m_{m}|+2}, ..., e_{t}\}\}$. 
We also normalize edge type weights in each independent sets following the formula:
\begin{equation}
\textit{$w_i^{*}$} = \frac{w_{i}}{\sum_{S(e_{i}) = S(e_{j})}w_{j}} 
\end{equation} 

%Second, within each independent edge set, edge-type weights are normalized to a probability distribution.

The second genetic approach is proposed based on the independent edge type sets and normalized edge type weights. Different from the first genetic approach, a `gene` here stores two values: a binary value $B$ to decide whether its related edge type is removed or kept and the normalized edge type weight calculated previously. 

In order to choose top $N$ edge types, for a `chromosome`,$N$ genes are with $B = 1$ and the rest $t-N$ genes have $B = 0$. binary values $B$ are exchanged in the Cross-over step, and the total number of genes with $B =1$ should be $N$ after the Mutation step, which means that each time a gene's binary value changes from 0 to 1, another gene should be randomly selected and its binary value changes from 1 to 0. When we calculate fitness score for a `chromosome`, only edge types (genes) with $B = 1$ are remained and their associated normalized weights $w$ are used to generate the PageRank ranking list $p(K)$ for all $K$ users. 

%The first two steps are preparations for the next secondary genetic algorithm step. Different from the previous genetic algorithm to generate edge type weight combination, a gene of current genetic algorithms refer to a type of selected edge, and its value is the edge-type weight calculated by the previous genetic algorithm. Therefore, a chromosome here refers to a combination of selected edge types. The number of genes refers to the number of edge types we want to choose.

To reach global optima faster, the initialization step of the second genetic algorithm uses a two-step sampling strategy including an edge type set selection process and an edge type selection process. 
 
% \[ \text{$P(S_{i})$} =
%   \begin{cases}
%   \frac{1}{M} , &   \text{$S_{i} \subseteq$ S}\\  0 , & \text{otherwise}\\
   
%   \end{cases}
% \]
% \begin{equation*}
% X \sim \mathcal{D}(S_{x})\, 
% \end{equation*}

First, one edge type set is randomly picked up from all independent edge-type sets following a uniform distribution. After a set $S_{1}$ is picked up, an edge type $e_{1}$ is selected based on its normalized edge-type weight. %This sampling process will continue unless  distinct edge types are selected.

%The rest of the steps are the same as previous genetic algorithms, including fitness function, selection, crossover, and mutation steps, which means initialized chromosomes are selected as pairs, processed via crossover and mutation steps, and, 

In the end, the `chromosome` with highest fitness score is returned as the final edge type selection result. And edge types with $B = 1$ are the selected top $N$ edge types which are remained in the heterogeneous graph. %salient edge-type combination which can best represent the entire heterogeneous graph. 

\begin{equation}
    Cost(u, S) = \sum_{s \in S}\mathbb{I}(G(u),G(s))\frac{C(u)*C(s)}{D(s|u)*\mu(\mathcal{N},\mathcal{C})^{2}} 
\end{equation}

C(u) and C(s) means the cluster size of user u and song s. $\mathcal{N}$ is the number of nodes in the graph, $\mathcal{C}$ is the number of communities. $\mu(\mathcal{N},\mathcal{C})$ is the average cluster size. D(s|u) is the preference degree of song s towards user u. $\mathbb{I}(u,s)$ is a judging function where:

\begin{equation}
  \mathbb{I}(G(u),G(s)) =
  \begin{cases}
    \alpha,       & \quad G(s) =  G(u)\\ 
    1-\alpha,  & \quad G(s) \neq  G(u)\\
  \end{cases}
  \label{eq:relu}
\end{equation}

$\alpha$ is from 0 to 1. G(s) refers to the community of s. 


